The Making of Cloud Applications An Empirical Study on Software Development for the Cloud

Cloud computing is gaining more and more traction as a deployment and provisioning model for software. While a large body of research already covers how to optimally operate a cloud system, we still lack insights into how professional software engineers actually use clouds, and how the cloud impacts development practices. This paper reports on the first systematic study on how software developers build applications in the cloud. We conducted a mixed-method study, consisting of qualitative interviews of 25 professional developers and a quantitative survey with 294 responses. Our results show that adopting the cloud has a profound impact throughout the software development process, as well as on how developers utilize tools and data in their daily work. Among other things, we found that (1) developers need better means to anticipate runtime problems and rigorously define metrics for improved fault localization and (2) the cloud offers an abundance of operational data, however, developers still often rely on their experience and intuition rather than utilizing metrics. From our findings, we extracted a set of guidelines for cloud development and identified challenges for researchers and tool vendors.

==> src/access_data.tex <==
% !TEX root = ../cloud-dev.tex


==> src/communication.tex <==
\subsection{Inter-Team Communication and DevOps}

\subsubsection*{Interview Observations}

In this section, we report on how communication between the roles of software development and operations engineering have changed through the cloud.

\subtitle{DevOps Communication} As discussed in Section~\ref{sec:bg}, it is often argued that cloud computing goes hand in hand with a DevOps style of communication, which leads to higher collaboration between software developers and operations engineers. In our interviews, this notion was not undisputed. While five interviewees (P9-P13) have agreed with the DevOps vision, the remaining participants (including most of our study participants from larger companies) have argued that there are still dedicated development and operations teams, and that there is still considerable friction between those teams:

\interviewquote{The back and forth with our performance team is [still] pretty time-consuming.}{P2}


%\interviewquote{Das hin- und her mit dem Performance Team ist schon zeitintensiv.}{Dev8}
%\interviewquote{Da wir in der Anwendungsentwicklung sind, sehen wir die Probleme so wie wir sie auch in traditionellen Sicht sehen würden.}{Dev7}
Interestingly, even companies that self-identify as following a DevOps approach still seem to generally have a separation between engineers that solely implement functional features, and engineers that mostly develop infrastructure code:%, and deal with operations concerns:

\interviewquote{We have our server/DevOps guy. (\ldots) He handles the whole monitoring and tools thing}{P9}

\subtitle{Infrastructure Transparency} Three of the DevOps participants (P9, P12 and P13) were also making use of IaC tooling for server management. They argue that this brings them transparency regarding their infrastructure:

\interviewquote{What happens in our infrastructure is a lot more obvious. Everything we do on that level [infrastructure] is over code  (\ldots) So, I don't need ask my colleague what he did to get that process running - I just look at the code and maybe the commit history}{P9}

\subsubsection*{Survey Results}

In the quantitative survey, there was a general agreement with these observations (cf. Figure~\ref{fig:survey_communication}). The survey responses show that, especially in large companies, communication and interaction has increased between application developers and operations engineers (72\%). 
Contrary to our interview study, the difference between the responses of developers working in smaller or larger companies in terms of collaboration between development and operations is not large. For smaller companies, 70-74\% tend to agree that their operations and development are now handled by the same staff, versus 57-60\% in larger companies. This data suggests that, even in larger companies, the gap between development and operations activities converges. 

%\pl{Figure \ref{fig:survey_communication} needs some sort of key for the numbers on the left-hand size. Also, the division here is not the same as in Section~\ref{sec:methodology}.}


\begin{figure}[h!] \centering
	\includegraphics[width=\columnwidth]{images/communication}
	\caption{Results regarding Team Communication grouped by company size (same key as in Figure \ref{fig:survey_releases})} 
	\label{fig:survey_communication}
\end{figure}

\resetObservations
\begin{observations}
\simpleobservation{C}{In the cloud, there is more collaboration between application developers and operations engineers}
\simpleobservation{C}{In smaller companies, operations and application development are often handled by the same staff}
\simpleobservation{C}{In larger companies, the separation between operations and application development is still intact}
\end{observations}

\subsubsection*{Discussion}

Based on our interviews and survey data, it seems that the notion of DevOps is indeed becoming a reality. Between half and 3 out of 4 developers state that cloud computing has brought them closer together with their operations team, and especially smaller companies are actively adopting the DevOps terminology and tooling (including IaC). However, quite contrary to the purist DevOps idea, our interviews have also shown that even small companies that self-identify as having a DevOps approach, still often think in silos of software developers and operation engineers. The main difference is that now these operators are referred to as ``DevOps engineers''. These engineers are rarely responsible for building functional features. Instead, their job is often to monitor performance (as discussed in Section~\ref{sec:data}) and maintain the IaC code for provisioning. 


==> src/impact_development.tex <==
% !TEX root = ../icse14.tex

\subsection{Impact on Application Development}

\subsubsection*{Interview Observations}

We found that developers face different kind of challenges, depeloynding on the cloud model they use. Thus, we further divide this section to address challenges developers have in either \emph{IaaS} or \emph{PaaS}. For more SaaS-oriented developers, actual application development has arguably not changed much (cf. Section~\ref{sec:def}).
% \emph{Note that:} The findings discussed in this section are thus not relevant for developers that view the cloud as a delivery model (SaaS).

%\subsubsection*{Application Development on IaaS}
\subtitle{Design for Failure in IaaS} A major impact that moving to the IaaS cloud brings about is that it forces developers to build highly fault-tolerant applications. IaaS providers reserve the right to shut down any resources at any time, on short or without prior notice:
\interviewquote{One interesting thing that is very cloud specific and influenced our architecture is, that the cloud provider tells you, we can kill your machine everytime we want.}{P9}
This makes any state change on a particular instance (that is not automated through a script or documented in any way) potentially dangerous, as any change may be lost when the instance is discarded by the provider.
 When developing on IaaS, instances come in various configurations for different purposes. Different parts of an application may have different requirements on the underlying hardware (e.g., CPU or I/O intensity) that can leverage the advantages of certain instance types. Interviewees deploying on IaaS reported that they enjoy the flexibility of "disposable instances" (P12) for partial deployments and redundancy:
\interviewquote{We have divided our application into many services. For one specific service we kill off and start new instances all the time, also to have proper redundancy.}{P9}

%Except for these points, development on IaaS platforms resembles traditional development practices. We observed a higher impact on  development practices in PaaS.

%\subsubsection*{Application Development on PaaS}
\subtitle{Higher Expectations in PaaS} In PaaS, developers expect the platform to handle certain operational aspects in combination with the software stack for them. Operational aspects include, for instance, variations in system load and fail-over/recovery of services and the underlying infrastructure.  What aspects the software stack handles differs among platform providers, but, generally speaking, includes a variety of middleware services that can be accessed through the platform's API. \\
\indent A recurring theme among interviewees developing on PaaS was that they do not care about system load, as they expect the platform to take care of scalability issues and provide elasticity out of the box. 

\subtitle{Design Restrictions} As already mentioned in Section \ref{sec:bg}, cloud platforms are only able to provide this convenient experience by imposing certain restrictions: (1) restrictions in the way developers can architect and design their solutions, (2) restrictions on technologies and libraries that can be used. However, to our interview participants, these restrictions were not all negative. Some developers feel that it allows them to focus more on delivering business value, instead of tinkering with low-level technology choices:

\interviewquote{But I don't wanna make those decisions [on application design and technology] anyway. (...) The cool thing - from a product design point of view - is, that you know what works on AppEngine and what doesn't}{P11}

% However, as P3 argues, even before PaaS, in larger companies the stack was already handled by a separate entity (e.g., a separate operations team), and the application developer had usually no say in it. That means that, especially in larger companies, the platform was already imposing certain restrictions anyway.
% \pl{I am not sure about this paragraph. I think this needs to be either removed or re-written.}

\subsubsection*{Survey Results}

We confirmed the observation that developers expect the cloud to handle load variations for them through our quantitative survey, and put the responses of IaaS versus PaaS developers in contrast (see Figure \ref{fig:variation_load}). 

%\pl{Why do more than 50 percent assume IaaS handles load for them?}

\begin{figure}[h!] \centering
	\includegraphics[width=\columnwidth]{images/variation_load}
	\caption{Results regarding expectations on system load handling (same key as in Figure \ref{fig:survey_releases})} 
	\label{fig:variation_load}
\end{figure}

%\pl{Label is cut in Figure \ref{fig:variation_load}}

Further, we asked survey respondents to list particular restrictions they encounter, which are specific to the cloud. 119 participants stated multiple restrictions, which we categorized and quantified in Table \ref{tab:restrictions}. More generally, we also asked  whether the survey respondents face limitations in application architecture and design. The results are in this regard inconclusive (with 51\% of disagreeing and 36\% agreeing). 

\begin{table}[h]
\caption{Most significant restrictions developers have encountered on cloud platforms} \label{tab:restrictions}
\begin{tabular}{ll}
 \textbf{Restrictions} & \% \\
\hline
Development Environment, SDK/API & 56\% \\
Technology \& Services (e.g., Language, Frameworks, Libraries) & 39\% \\
Distributed Architecture (Stateless, High Availability Design) &  31\% \\
Data Storage, Persistence                     & 27\%  \\
%High Availability Design (e.g. Fault-tolerance, Recovery)   &  13\% \\
\hline
\end{tabular}
\end{table}

%\begin{figure}[h!] \centering
%	\includegraphics[width=\columnwidth]{images/limited_architecture}
%	\caption{Results regarding limitations in architecture and design of cloud applications} 
%	\label{fig:limited_architecture}
%\end{figure}
	
\resetObservations	
\begin{observations}
\simpleobservation{D}{Developers expect that the cloud automatically handles variations in the system load}
\simpleobservation{D}{Cloud platforms restrict the way how developers architect and design their solutions}
\simpleobservation{D}{For some developers, restrictions are not always perceived as negative, as they allow them to focus on delivering (business) value}
\simpleobservation{D}{Developers on the (IaaS) cloud need to design for fault-tolerance due to the possibility of sudden instance termination}
\end{observations}	
	
\subsubsection*{Discussion}

%Unsurprisingly, 80\% of survey respondents deploying on PaaS confirm that the cloud automatically handles increasing system load for them.
In the following, we briefly discuss the results of the quantitative survey.

\subtitle{Load Handling in IaaS}  Surprisingly, even on IaaS, 54\% agree that the cloud automatically handles variations in system load for them, although this is not an inherent feature of IaaS solutions. Developers agreeing with this statement might refer to the ease of acquiring server instances that enables the handling of increasing system load through horizontal scaling. Furthermore, IaaS vendors sometimes offer dedicated load balancing instances (e.g., Amazon's Elastic Load Balancer) that facilitate these capabilities.

\subtitle{Limitations in Design \& Architecture} Survey respondents are somewhat indifferent, but generally disagree that the cloud limits possible architectures and designs. A possible explanation to this result is that developers may feel that they were restricted in non-cloud environments as well (e.g., through either frameworks or middleware). However, restrictions do exist in the cloud, as 119 respondents stated particular (sometimes multiple) restrictions. Unsurprisingly, the most cited restrictions were the adherence to a certain development environment (including an SDK or API), and supported technologies by the cloud platform. 

\subtitle{Distributed Architecture} On the other hand, the focus on a distributed architecture (i.e., stateless/share-nothing approach, focus on fault-tolerance) was mentioned less than we would have expected based on our interviews. Explanations of this result could be two-fold: (1) developers do not see these architecture considerations as too much of a restriction, as it enforces good practice and results in high availability and scalability, (2) some developers do not build (or do not need to build) distributed architectures. 

% \subtitle{Ephemeral Storage} Persistence of files and data must be handled differently due to ephemeral storage on cloud platforms (i.e., instances can be replaced with a newly provisioned instance). However, this issue has been addressed by cloud vendors by providing storage capabilities (databases, file storage) as a service.
%\footnote{Amazon S3, Google Cloud Storage, ...}.



==> src/method.tex <==
%!TEX root =../icse14.tex

\section{Research Method}
\label{sec:methodology}

To investigate how the cloud changes software development practices, we conducted a study based on techniques found in Grounded Theory~\cite{hoda:12}. Following the recommendations in~\cite{bratthall:02}, we used a mixed methodology consisting of three steps of data collection and iterative phases of data analysis. First, we determined a set of 23 open-ended questions for a \emph{qualitative interview study} based on our research questions. We interviewed 16 participants working in 5 companies of varying size located in three countries in Europe and the United States. 
%Through coding and analyzing the interview transcripts, we identified 20 observations. 
To further substantiate these observations, we ran a \emph{quantitative survey}, for which we gathered responses from 294 professional software developers. We performed open coding on the open ended questions in the survey to identify major differences between cloud and non-cloud development that are of high interest. We identified 4 topics of high interest, that guided the last step of our data collection phase, a \emph{qualitative deep-dive interview study} to allow for more profound insights. 
%Our 13 participants for this second set of interviews work in companies of different sizes and which are located in Germany, Austria, the Netherlands, and the United States. After coding and analysing the results of our interview study, we identified 11 observations, which we then validated based on a larger-scale \emph{quantitative validation survey}. The survey attracted a total number of 249 respondents.
%Based on the collected data, we were able to validate 8 of the observations formed during the interview study.
All interview materials and survey questions can be found on our web site\footnote{http://www.ifi.uzh.ch/seal/people/cito/cloud-developer-study.html}. 
%Supplementary material for our study including the inte (i.e., interview and survey questions) are available online\footnote{TODO}.
%\pl{Fix footnote.} 

%\subsection{Exploratory Interviews}
%\label{sec:relatedworkstudy}
%Study of related work and brainstorming sessions were employed to derive the initial interview topics that would allow to cover all areas we need to answer the research questions.
%\textbf{Protocol.} To guide our research, we conducted exploratory interviews with a small number of experienced cloud developers. In these interviews, the first author of this paper asked and discussed participants' perceptions of cloud projects, and how these differ from other projects, both within their company and more generally. These interviews were guided by a list of topics rather than concrete questions. Interviews were conducted in German, lasted approximately 45 minutes each, and were audio-recorded.

%\textbf{Participants.} We interviewed three experienced developers from a large German software house. Our participants in this phase had 24, 16, and 4 years of professional experience, and were at the time of the interview all involved in cloud-related projects.

%\textbf{Analysis.} Based on the results of these interviews, and the personal experience of the authors of this paper, we drafted and iteratively refined a set of questions and themes for a larger, more formal, qualitative interview study. The main themes identified were ``changes in  processes and communication'', ``necessary changes and restrictions in application design'', ``utilization of cloud-based tools'' (e.g., Web-based IDEs) and ``availability of runtime data''.   

\subsection{Qualitative Interview Study}
\textbf{Protocol.} We conducted semi-structured interviews with software developers that previously already deployed software in the cloud in a professional context. We covered all questions with each participant, but the concrete order of questions followed the ``flow'' of the interview. Interviews were conducted by the first author, either face-to-face on-site of the interviewee or via Skype. Interviews lasted between 30 and 60 minutes, were conducted in either German or English, and were audio-recorded.

\textbf{Participants.}
%   Finally, the study was conducted with 16 participants, all male, software developers that have deployed in a cloud infrastructure  on a professional level. 10 participants were employed by two enterprise companies (Germany, New York/USA), 6 by SMEs (Austria, Netherlands, Boston/USA). Interviews lasted between 30 and 45 minutes and were conducted in person by the first author if possible; only 1 of the interviews was conducted over Skype. 2 interviews were conducted with 2 participants at once due to participants' time constraints.
Interview participants were recruited from industry partners and our personal network. To cover a broad range of cloud development experiences, we recruited participants from both, smaller companies (1 -- 100 employees) and larger enterprises ($>$ 100 employees). Participants had to either deploy on IaaS or PaaS as well as in public and private clouds. Furthermore, we also made sure to recruit some participants that delivered SaaS applications. 

Overall, we recruited 16 participants, all male software developers with an average professional development experience of 7 years ($\pm$ 5 standard deviation) from 4 different countries and two continents (see Table \ref{tab:participants}).
%Participants P6, P7 and P8 are not part of the interview study, as those were used in the exploratory phase of our research.

\begin{table}[h] \centering
\caption{Qualitative Interview Participants}
\label{tab:participants}
\scriptsize{
\begin{tabular}{|l|l|l|}
 \hline
 \textbf{Participant} & \textbf{Platform}  & \textbf{Experience (Years)} \\
 \hline
 \rowcolor[HTML]{EFEFEF} 
 \multicolumn{3}{|l|}{Company A, Team 1, European Country 1 (Enterprise)}
 \\
 \hline
 P1  & PaaS & 14\\
 P2  & PaaS & 20\\
 P3  & PaaS & 5\\
 P4  & PaaS & 6\\ 
 \hline
 \rowcolor[HTML]{EFEFEF} 
 \multicolumn{3}{|l|}{Company A, Team 2, European Country 1 (Enterprise)}
 \\
 \hline 
 P5  & PaaS & 6\\
 P6  & PaaS & 3\\
 P7  & PaaS & 23\\
 P8  & PaaS & 11 \\
 \hline
 \rowcolor[HTML]{EFEFEF} 
  \multicolumn{3}{|l|}{Company B, European Country 2 (Small Company)}
 \\
 \hline  
 P9  & IaaS & 5\\
 \hline
 \rowcolor[HTML]{EFEFEF} 
 \multicolumn{3}{|l|}{Company C, European Country 3 (Small Company)}
 \\
 \hline 
 P10  & PaaS & 4\\
 P11  & PaaS & 3\\
 \hline
 \rowcolor[HTML]{EFEFEF} 
 \multicolumn{3}{|l|}{Company D, USA (Small Company)}
 \\
 \hline  
 P12  & IaaS & 6 \\
  \hline
 \rowcolor[HTML]{EFEFEF} 
 \multicolumn{3}{|l|}{Company E, USA (Enterprise)}
 \\
 \hline 
 P13  & IaaS & 5 \\
 \hline
 \rowcolor[HTML]{EFEFEF} 
 \multicolumn{3}{|l|}{Company A, Team 3, European Country 1 (Enterprise)}
 \\
 \hline 
 P14 &  PaaS & 16\\
 P15  & PaaS & 4\\ 
 P16  & PaaS & 24\\
 \hline  
\end{tabular}
}
\end{table} 

\textbf{Analysis.} After the interviews, all audio recordings were transcribed. The first two authors then used an open coding technique to iteratively code and categorize participants' statements, resulting in a set of 20 observations. All observations are supported by statements of multiple interview participants. Due to the inherent heterogeneity of our interviewees, some of these observations relate mostly to developers working in either smaller or larger companies, or with specific cloud models (e.g., IaaS or PaaS).
% since there is a difference between developers deploying on IaaS or PaaS technologies. 

% \subsubsection{Protocol}
% 
% We started off by asking an open-ended and deliberately ambiguous question: 'How is developing applications in the cloud different from developing in a traditional environment?'. As expected, this question sparked a discussion on what the 'cloud' actually is, and what 'traditional' means.
% 
% Afterwards, we addressed each of the topics we derived in the previous phase (see Section \ref{sec:relatedworkstudy}). We followed up on aspects we seemed were interesting and would probably yield new insights. 
% Finally, we thanked the developer and expressed our gratitude with Swiss chocolate. We informed them of our future work with the data and asked for permission to contact them again for clarification that might be needed during the coding and analysis phase. The interviews were voice recorded and then transcribed.
% 
% \subsection{Coding \& Analysis}
% In the third phase, we employed open coding, iterating through our interview transcripts first extracting categories from statements. In further iterations we extracted codes and formulated hypothesis and findings that we report in Section \ref{sec:findings}.

\subsection{Quantitative Survey}

\textbf{Protocol.} In the second step of our study, we designed a survey with 32 questions, most of which directly map to the observations. The questions were primarily formulated as statements, asking participants to state their agreement on a Likert scale. 
To target developers with experience in cloud technologies, we mined email addresses of GitHub\footnote{http://www.github.com} users that ``follow'' a repository of a number of popular cloud platforms, including Amazon Web Services, Heroku, Google Cloud Platform, CloudFoundry, and OpenStack. We then discarded all users without a public email address in their profile, and contacted the remaining users with a description and link to our online survey. To motivate developers to participate in the survey, we held a raffle for all participants to win one of two 50 USD Amazon gift vouchers. The survey was in English, and took an average of 12.2 minutes to complete.

\textbf{Participants.} We emailed the survey invitation to 2000 GitHub users. We gathered a total of 294 responses (response rate of 14.7\%). Of all 294 participants, 192 were employed in smaller companies (between 1 and 100 employees) and 102 were employed in large companies. 71\% stated their job role as software developers, 22\% as team lead or product owner, 4\% as operations engineers, and the remaining 3\% listed software architect, researcher or chief technology officer (CTO). The average professional development experience per participant was 8.8 ($\pm$ 5.9) years.

\textbf{Analysis.} 
We analyzed the distributions of Likert responses and present the results along with the according observations from the interview study phase. Furthermore, we examined the responses of three free-text questions on overall differences in development in cloud versus non-cloud environments, tooling, and restrictions in the cloud. Based on these results, we were able to enhance our understanding of some of the observations. In some cases, we gained new insights that led to the formulation of further observations.

\subsection{Qualitative Deep-Dive Interviews}
\textbf{Protocol.} Through the examination of open-ended survey questions, we identified 4 topics of high interest: (1) Fault localisation, (2) Monitoring \& Performance Troubleshooting, (3) Cost of Operation, and (4) Design for Scalability. In order to get more profound insights into these topics, we conducted another round of deep-dive interviews. We followed the same protocol as in the first round of qualitative interviews.

\textbf{Participants.}
Interviewees were recruited through our personal network. Interviews were again conducted by the first author, lasted between 30 and 45 minutes and were audio-recorded.

Overall, we recruited 8 participants, 7 male and 1 female software developers with an average professional development experience of 9.2 years ($\pm$ 7 standard deviation) from 6 different countries and two continents (see Table \ref{tab:deep_dive_participants}). All participants were from different companies.
%Participants P6, P7 and P8 are not part of the interview study, as those were used in the exploratory phase of our research.

\begin{table}[h] \centering
	\caption{Qualitative Deep-Dive Interview Participants}
	\label{tab:deep_dive_participants}
	\scriptsize{
	\begin{tabular}{|l|l|l|}
		\hline
		\textbf{Participant} & \textbf{Platform}  & \textbf{Experience (Years)} \\
		\hline
		D1  & PaaS & 4\\
		D2  & IaaS/PaaS & 7\\
		D3  & IaaS & 20\\
		D4  & IaaS & 15\\
		D5  & IaaS & 14\\
		D6  & IaaS & 8\\
		D7  & PaaS & 1\\
		D8  & PaaS & 6\\
		D8  & IaaS & 5\\
		\hline
	\end{tabular}
}
\end{table} 

\textbf{Analysis.} During our analysis of the deep-dive interview data, we associated recurring themes to the existing data we gathered in the previous two phases to allow for more profound insights into the difference between cloud and non-cloud development. All observations are supported by multiple statements of the interview participants.


%\tf{The following is a summary of the results, not the way you analyzed the data! Please change, i.e. state what you did to analyse the results} Statistical analysis of the responses of our survey led to the validation of 8 of our interview observations. 2 observations had to be discarded based on the survey data. Further, we were able to enhance our understanding of some of the observations, based on free-text feedback given in the survey by a subset of the participants. %\textbf{TODO:} this should be formulated much more exact.

==> src/process_communication.tex <==
% !TEX root = ../cloud-dev.tex
% TODO: add how releases have evolved, with division in company size

% \subsection{Process, Communication, and Team Dynamics}

\subsection{RQ1: How does the development process change in a cloud environment?}

In this section, we report on how cloud development has affected the software development process. We organize this section as follows to relate our findings with a standard development process \cite{[sommerville:software_engineering]}: (1) Project Management Methodology and Release Management, (2) Design \& Architecture, (3) Implemention, Integration \& Testing, (4) Deployment \&Automation, and (5) Troubleshooting \& Maintenance.

\subsubsection{PM Methodology and Release Management}

\subheading{Agile Process} All interviewees across the board described their development process as agile. The majority of the participants reported having SCRUM as their process model, while two interviewees working for smaller companies reported using Kanban. P3 went as far as to state that \emph{``SCRUM got introduced in the cloud"}.

\subheading{Release Management} Due to the combination of agility and the cloud, releases become more frequent and changes reach the customer faster. More frequent releases also led to customers starting to expect quicker reaction to change requests:
\interviewquote{What changed a lot are the expectations due to the faster release cycles.}{P2}
%\interviewquote{Was sich sehr verändert hat, ist die Erwartungshaltung durch die schnelleren Releasezyklen.  Es gab ne Zeit da haben wir nach dem Prinzip “Works as designed” gearbeitet, das wurde dann geändert auf “Works as expected”.}{Dev2}

However, what ``more frequent" means still depends on the company and its processes. Enterprise companies reported that they have moved from releasing less than once a year to multiple times per year: 
\interviewquote{We released very rarely compared to the cloud. [Now] we have a lot more releases per year, sometimes 4-5, before that maybe once a year.}{P5}

On the other hand, interviewees at companies which follow a continuous delivery approach, reported releasing multiple times per day.

In our quantitative survey, we wanted to analyze the possible correlation of cloud development and agile processes. We asked participants about the process they use now, and the process they used before moving to the cloud. 86\% of respondents agree to using an agile process now, but 77\% of respondents also state that they were using an agile process even before moving to the cloud. Nevertheless, a majority of respondents (73\%) agree that their process is now more agile than before moving to the cloud.\\
\indent The survey concurs with most of our findings regarding shorter release cycles (70\%), (2) faster feature delivery, (3) quicker reaction to customer demands.
However, when it comes to higher customer's expectations, only 49\% agreed with the finding, while 37\% were neutral on the topic.

%\begin{figure}[h!] \centering
%	\includegraphics[width=\columnwidth]{images/releases}
%	\caption{Results regarding Release Management} 
%	\label{fig:survey_releases}
%\end{figure}

\resetObservations
\begin{observations}
 \simpleobservation{B}{For some developers, the cloud has led to the adoption of a more agile development process}
% \observation{Changes reach the customer faster in the cloud}
 \simpleobservation{B}{Releases become more frequent in the cloud, and changes reach the customer faster}
 %\simpleobservation{B}{Customers of cloud services expect quicker reaction to changes and more frequent releases}
 \simpleobservation{B}{For some, customers of cloud services expect quicker reaction to changes and more frequent releases}
\end{observations}

%\subsubsection*{Discussion}

%Through the findings of our interview study, we hypothesized a possible causality between cloud development and agile processes. Our observation that the cloud has led to a more agile process has been confirmed by the quantitative survey. However, there are some issues that need to be addressed. Firstly, most of the participants have already had an agile process before moving to the cloud, so there is no definitive way of inferring causality. Secondly, different developers might have different notions of what ``agile'' actually means. This might skew results in one way or another. %Overall, the results of the validaton survey on this topic are relatively inconclusive.
%Additionally, while shorter release cycles have been a major theme in the interview study, it is not quite clear whether this has been facilitated by the cloud, DevOps, more agile processes, or a combination of all of those topics. 
%However, automation in the deployment process (see Section \ref{sec:tooling}) might ...



\subsection{Inter-Team Communication and DevOps}

\subsubsection*{Interview Observations}

In this section, we report on how communication between the roles of software development and operations engineering have changed through the cloud.

\subtitle{DevOps Communication} As discussed in Section~\ref{sec:bg}, it is often argued that cloud computing goes hand in hand with a DevOps style of communication, which leads to higher collaboration between software developers and operations engineers. In our interviews, this notion was not undisputed. While five interviewees (P9-P13) have agreed with the DevOps vision, the remaining participants (including most of our study participants from larger companies) have argued that there are still dedicated development and operations teams, and that there is still considerable friction between those teams:

\interviewquote{The back and forth with our performance team is [still] pretty time-consuming.}{P2}


%\interviewquote{Das hin- und her mit dem Performance Team ist schon zeitintensiv.}{Dev8}
%\interviewquote{Da wir in der Anwendungsentwicklung sind, sehen wir die Probleme so wie wir sie auch in traditionellen Sicht sehen würden.}{Dev7}
Interestingly, even companies that self-identify as following a DevOps approach still seem to generally have a separation between engineers that solely implement functional features, and engineers that mostly develop infrastructure code:%, and deal with operations concerns:

\interviewquote{We have our server/DevOps guy. (\ldots) He handles the whole monitoring and tools thing}{P9}

\subtitle{Infrastructure Transparency} Three of the DevOps participants (P9, P12 and P13) were also making use of IaC tooling for server management. They argue that this brings them transparency regarding their infrastructure:

\interviewquote{What happens in our infrastructure is a lot more obvious. Everything we do on that level [infrastructure] is over code  (\ldots) So, I don't need ask my colleague what he did to get that process running - I just look at the code and maybe the commit history}{P9}

\subsubsection*{Survey Results}

In the quantitative survey, there was a general agreement with these observations (cf. Figure~\ref{fig:survey_communication}). The survey responses show that, especially in large companies, communication and interaction has increased between application developers and operations engineers (72\%). 
Contrary to our interview study, the difference between the responses of developers working in smaller or larger companies in terms of collaboration between development and operations is not large. For smaller companies, 70-74\% tend to agree that their operations and development are now handled by the same staff, versus 57-60\% in larger companies. This data suggests that, even in larger companies, the gap between development and operations activities converges. 

%\pl{Figure \ref{fig:survey_communication} needs some sort of key for the numbers on the left-hand size. Also, the division here is not the same as in Section~\ref{sec:methodology}.}


\begin{figure}[h!] \centering
	\includegraphics[width=\columnwidth]{images/communication}
	\caption{Results regarding Team Communication grouped by company size (same key as in Figure \ref{fig:survey_releases})} 
	\label{fig:survey_communication}
\end{figure}

\resetObservations
\begin{observations}
\simpleobservation{C}{In the cloud, there is more collaboration between application developers and operations engineers}
\simpleobservation{C}{In smaller companies, operations and application development are often handled by the same staff}
\simpleobservation{C}{In larger companies, the separation between operations and application development is still intact}
\end{observations}

\subsubsection*{Discussion}

Based on our interviews and survey data, it seems that the notion of DevOps is indeed becoming a reality. Between half and 3 out of 4 developers state that cloud computing has brought them closer together with their operations team, and especially smaller companies are actively adopting the DevOps terminology and tooling (including IaC). However, quite contrary to the purist DevOps idea, our interviews have also shown that even small companies that self-identify as having a DevOps approach, still often think in silos of software developers and operation engineers. The main difference is that now these operators are referred to as ``DevOps engineers''. These engineers are rarely responsible for building functional features. Instead, their job is often to monitor performance (as discussed in Section~\ref{sec:data}) and maintain the IaC code for provisioning. 


==> src/relevant_metrics.tex <==
% !TEX root = ../cloud-dev.tex
\subsubsection{Types of Relevant Metrics}
\label{sec:data}

%Ultimately, the purpose of tooling in software engineering is to either provide automation of manual tasks or to provide data to aid the developer in the software evolution process. In the latter case,

% Ultimately, one of the purposes of tooling in software development is to provide data to aid the developer in the software evolution process. Developers leverage various types of data to incrementally evolve their software and guide them through debugging. Given that

\subheading{Access to Data and Metrics}
In general, interviewees expressed that now they have more metrics on production systems available, as well as that they look at more metrics than before they moved to the cloud:
\interviewquote{Especially now in the cloud (with Heroku or Amazon) they provide so much data. Putting this data in a graphing tool and looking at it once in a while has become increasingly easier.}{P12}
%Orig: Speziell in der Cloud (mit Heroku oder Amazon) die haun sowieso so viele Daten raus. Das einfach in ein Graphing tool reinhauen und sich das hin- und wieder mal ansehen ist echt keine Hexerei

From the quantitative survey, we see that the majority of survey respondents (71\%) state that they look at more metrics than in non-cloud environments. We can also see that 62\% actually have more metrics available than before (see Q11 and Q12 in Figure \ref{fig:findings}).

\subheading{Organizational Limitations} Five interviewees reported that, when trying to find the root cause of a bug, obtaining production logs has become harder than in non-cloud environments. However, the difficulty in these cases did not arise from technical limitations, but rather from limitations of organizational nature:
\interviewquote{You need an approval from your manager, then from the customer, who reviews the whole process (...) It's all very conservative}{P6}
In these particular instances, customers expressed privacy concerns they had with cloud platforms leading to higher rigor in organizational processes to obtain any kind of data from production systems. 

%A possible causality between the two figures is discussed later on.

\subheading{Production Data} Access to production data has become easier according to survey respondents. For developers on PaaS systems, access to production systems is probably seen as easier because platform providers aim on offering a holistic solution to cloud developers. In IaaS, the majority of respondents were neutral on the topic. This is because, in this cloud model, access to the systems is unchanged compared to non-cloud environments.
Our original observation was derived from interviewees within a certain company and probably originated more from specific company policies, rather than being inherent to cloud development.

\subheading{Metric Inspection} The quantitative survey confirms our observation on the higher availability of metrics, as well as the increase in inspection of metrics.
However, it is not clear whether developers now look at more metrics simply because more metrics are available in cloud environments, or whether developers actually need this data for their work.


Cloud platforms allow access to a variety of data\cite{vaquero:11}.  Hence, we asked our interviewees about what kind of data they look for while developing or debugging applications, and what the process of obtaining that data looks like.
We identified four types of data that are the most relevant to developers: (1) application-level performance, (2) load (e.g., throughput), (3) functional usage (e.g., how often a feature or method has been used), and (4) cost of operation. We prompted our interviewees on these types of data, and how they utilize them. %Additionally, we asked our survey respondents which of the metrics they use on a regular basis.
%Furthermore, we wanted to know how developers obtained these data artifacts.

\subheading{Performance and Load} Performance metrics were deemed to be of high importance among interviewees. Load metrics, on the other hand, if observed at all, were only interesting in combination with performance. Five of the interviewees (P3, P4, P8, P9, P11) also reported that when a performance issue is reported, they first try to identify the bottleneck by going by their gut feeling, rather than relying on data.
Access to performance and load metrics, however, differed greatly among participants. Some used dashboards which have all needed information instantly available, while others were reliant on weekly reports from a separate performance team. 

\subheading{Functional Usage} When prompted on functional usage data, all interviewees found it interesting, but most reported that they do not have access to such a metric. The most expressed opinion was that it is probably of more interest to the product owner than to developers. However, four developers (P3, P5, P6, P10) said it would be important to prioritize application features, both for maintenance and development purposes (e.g., knowing which bug to fix first based on how many users use a certain feature as opposed to another feature): 
\interviewquote{I would like to see how often has an action been executed per day. (\ldots) It would help to know what is only used by 10\%, [of the users] so we know we don't have to optimize it urgently}{P6}
%In our quantitative survey 58\% of users reported using functional usage on a regular basis.

\subheading{Cost of Operation} To most of our interviewees, the cost of operations (especially of specific code changes) are not a tangible factor. Some interviewees argued that having this information more wide-spread would be interesting to them, but does not fall into their responsibilities:
\interviewquote{I have no idea about the costs. I can just read it in the logs sometimes that in production we spawned 20-30 servers. It would be interesting to know, but it’s not really important for application development}{P5}

\subsubsection*{Survey Results}

Performance metrics enjoyed the same popularity among survey respondents as in the interview study, with 84\% agreeing on using it on a regular basis. Surprisingly, 76\% of survey respondents reported looking also at load at a regular basis, going against our observation in the interviews. \\
\indent Contrary to our observations in the interview study, in the quantitative survey (cf. Figure \ref{fig:log_access}), only 25\% deploying in an IaaS environment and 15\% deploying in a PaaS environment said that access to production data has become harder than in non-cloud environments. Many respondents were neutral on the topic, and 58\% of developers on PaaS said access has even become easier for them.

\begin{figure}[h!] \centering
	\includegraphics[width=\columnwidth]{images/log_access}
	\caption{Results regarding access to production data from the quantitative survey (same key as in Figure \ref{fig:survey_releases})} 
	\label{fig:log_access}
\end{figure}

Regarding costs of operation, 56\% indicated that they look at costs on a regular basis.

%Regarding costs of operation, particularly developers in small companies, as well as product owners in larger companies, care about the additional cost caused through new features or implementation decisions. From the quantitative survey, 56\% indicated that they look at costs on a regular basis.

%\resetObservations
%\begin{observations}
%\simpleobservation{F}{More metrics on production systems are available in the cloud}
%\simpleobservation{F}{Cloud Developers look at more metrics on production systems than before}
%\simpleobservation{F}{When trying to identify the root cause of a bug, access to production data has become easier}
%\simpleobservation{F}{Performance is deemed to be the most important metric cloud developers look at on a regular basis}
%\simpleobservation{F}{Functional usage is interesting to cloud developers, but only to prioritize feature/bug-fix requests}
%\simpleobservation{F}{Cost of operation is not a tangible factor to cloud developers}
%\end{observations}


==> src/underlying_cause.tex <==
Through our study we were able to find answers to our research questions to help identify how development practices have changed in the cloud.
After reflecting about our results, we found that many of the findings are related two major underlying causes: (1) \emph{Infrastructure at Scale} and (2) \emph{Volatility of Cloud Instances}.

We will now briefly explain these two causes and, where applicable, refer to them when presenting our findings in the following sections.

\paragraph{Infrastructure at Scale}
Infrastructure at Scale refers to the ability to spawn up many compute instances over an API. This ability sets up the need for more automation on many levels, including infrastructure, environment and test. 


\paragraph{Volatility of Cloud Instances}

Infrastructure (i.e., cloud instances) can be started up and shut down for various reasons. This volatility happens either through (1) the cloud provider, (2)  the load balancer, and (3) application logic. The cloud provider
(e.g., based on traffic patterns)
(a dynamically allocated instance finished the work it was supposed to do).




